Optimal Local Bayesian Differential Privacy over Markov Chains

In the literature of data privacy, differential privacy is the most popular model. An algorithm is differentially private if its outputs with and without any individual's data are indistinguishable. In this paper, we focus on data generated from a Markov chain and argue that Bayesian differential privacy (BDP) offers more meaningful guarantees in this context. Our main theoretical contribution is providing a mechanism for achieving BDP when data is drawn from a binary Markov chain. We improve on the state-of-the-art BDP mechanism and show that our mechanism provides the optimal noise-privacy tradeoffs for any local mechanism up to negligible factors. We also briefly discuss a non-local mechanism which adds correlated noise. Lastly, we perform experiments on synthetic data that detail when DP is insufficient, and experiments on real data to show that our privacy guarantees are robust to underlying distributions that are not simple Markov chains.

==> Pufferfish Privacy for Sanitized Databases/introduction-6-7-8pm.tex <==
\section{Introduction}
In the literature of privacy, differential privacy (DP)~\cite{dwork2014algorithmic} is the gold standard. An algorithm is differentially private if its outputs with and without any individual's data are indistinguishable. But there are numerous settings in which the semantic guarantees of differential privacy either aren't meaningful or are insufficient. Bayesian differential privacy (BDP)~\cite{yang2015bayesian} is a strict generalization of differential privacy that is applicable in many of these settings. However, BDP is more technically challenging to work with; our main theoretical contribution is providing a mechanism for achieving BDP when the data is drawn from a binary Markov chain. In this regard, we improve on the state-of-the-art BDP mechanism and show that our mechanism provides the optimal noise-privacy tradeoffs up to negligible factors. We also consider a mechanism which adds \textit{correlated} noise to the data, but find no improvement to noise-privacy tradeoffs. Lastly, we perform experiments on synthetic data that details when DP is insufficient, and experiments on real data to show that our mechanism works well in practice even when the underlying distribution is not a simple Markov chain. We start by arguing the need for stronger privacy than DP.

\subsection{Privacy Definitions}

Differential privacy forms privacy guarantees \textit{without} a model for how the data is generated. A differentially private mechanism guarantees that the probability ratio of observing any single output by applying the mechanism to two \textit{neighboring} databases is small, where two databases are neighbors if they differ in exactly one data point. Importantly, the probability here is only taken over the randomness of the mechanism, since there's no model for data generation. However, if an adversary has reasonable background knowledge regarding the data distributions, it may be the case that an $\eps$-differentially private mechanism will produce an output that is disproportionately more likely given one of two neighboring datasets. So in examples where adversaries can reasonably infer the data correlation model (e.g. US census data), differential privacy will \textit{not} prevent these adversaries from learning tuples. 

This limitation of DP is well understood;~\cite{dwork2014algorithmic} reframes this limitation in terms of the \textit{semantic} guarantee that DP provides. Suppose you are a medical researcher tasked with convincing users to divulge sensitive health data, which will then be published online. Differential privacy, according to the semantic interpretation, can be used as a \textit{tool} to encourage participation. Individuals, who can only control their own participation in the study, know that they will receive minimal harm \textit{directly tied} to their participation in the study. Viewed this way, DP is an entirely end-user focused persuasive tool. However, an ethical researcher would not only like to persuade users to participate, but also to understand and limit the harms caused by the study itself. DP answers the question of whether a single user ought to participate; BDP answers the question of whether the study ought to be performed. Put this way, BDP and similar privacy frameworks can be viewed as mechanism design for social good. Another way to frame this is that BDP persuades the researcher to publish their collected data, by more comprehensively limiting the harms to any study participant.

When the database consists of records that each belong to different individuals, DP can still be a reasonable choice (e.g. if the study could significantly help the participants). However, when considering data from a single individual, such as the mobility data of a single person, DP does not provide any meaningful guarantees. The distinction here is most salient when comparing which adversaries DP and BDP protect against. Suppose we are trying to protect Alice's time series data. Differential privacy guarantees \textit{only} that someone who knows Alice's location at all but one time step will not learn very much by analyzing the sanitized data set (their posterior after seeing the sanitized data won't change much)~\cite{yang2015bayesian}. BDP guarantees that regardless of how much the adversary knows, they won't learn much by analyzing the sanitized data set. Presumably, Alice is not interested in protecting her data only against an adversary who knows almost all of it. Analogously, our privacy guarantee should not depend on how many data points the adversary knows.\footnote{Notice that when the data at each time step is independent, BDP reduces to DP; the adversary's knowledge of Alice's location at time $x_i$ is irrelevant to their knowledge of Alice's location at time $x_j$.}

\subsection{Our Contribution}

BDP is an instantiation of the Pufferfish privacy framework~\cite{kifer2014pufferfish}, a broad framework that allows us for customizable, robust privacy guarantees. We focus on providing \textit{non-interactive} mechanisms, which return ``sanitized'' (i.e. noisy) estimates of the real database. These are called non-interactive since the sanitized databases can be queried offline without further privacy loss; in contrast, query-based mechanisms must be rerun with additional privacy losses for each query. Our primary mechanism adds independent noise to each state; because of this, our mechanism achieves \textit{distributed}, or local, privacy guarantees. This means that no centralized curator need have access to the agents' true data. Instead, the owners of each tuple can privately sanitize their entry before submission. When privacy guarantees are framed in terms of trust or persuasive power, this property is extremely attractive.\footnote{Though we mostly focus on the setting where every tuple belongs to one individual, our mechanism is still applicable to the conventional setting.} 
% The main challenge in the setting of correlated data is a lack of suitable mechanisms. Recent advances~\cite{song2017pufferfish} provide a Pufferfish private mechanism under the query setting: given a functional query, e.g., counting the number of smokers, the mechanism's report is private and close to the real value. That mechanism has two main limitations: (1) it is computationally intractable, and (2) the mechanism cannot handle adaptive queries, but instead must be rerun (and lose additional privacy guarantees) for each query. For this reason, we design efficient \textit{non-interactive} mechanisms, that will release a noisy estimate of the real database (to make the reports reusable).

Our model is relatively simple; we represent data correlations via Markov chains, and these preliminary results consider only binary state spaces. We assume that the data is \textit{positively} correlated, as in the case of location data, where an individual is more likely to stay in the same location than leave (given a fine-enough time scale). 
\paragraph{Roadmap} In Section 2, we review the definition of BDP, and apply it to the context of our problem. In Section 3, we first state our main theorem, which describes the noise-privacy tradeoffs of our mechanism. We show that $\eps$-differential privacy requires less noise than $\eps$-BDP, but also experimentally evaluate how much privacy degrades when an adversary has knowledge about the data distribution. (show concrete attack on DP with synthetic data). We then compare our noise-privacy tradeoffs with previous results, showing that we improve on the state-of-the-art. To round out our experiments, we evaluate our mechanism on real heart rate data, showing that the Markov chain modelling assumption cannot be exploited by an LSTM deep learning adversary. We also measure the accuracy of basic metrics on the sanitized data.

In Section 4, we prove our main theorem and also briefly discuss a mechanism which adds \textit{correlated} noise to the data. We find no improvement to the noise-privacy tradeoff, but \todolong{add some stuff about uses of the correlated noise mechanism, or say that it shows that our independent noise mechanism optimizes over a far large space of mechanisms.}

\subsection{Related Work}
In recent years, there have been many correlation-aware privacy definitions. We discuss a few of the most relevant definitions. Most of the definitions are instantiations of Pufferfish privacy ~\cite{kifer2014pufferfish}, a broad Bayesian framework. The most relevant is obviously Bayesian differential privacy, initially proposed by Yang et al.~\cite{yang2015bayesian}. They show that BDP is a very natural way to formulate a stronger privacy guarantee than DP, as BDP simply quantifies over adversaries with knowledge of any tuples, while DP only protects over adversaries who know all but one tuple. Zhao et al. consider an equivalent formulation that they term dependent differential privacy (DDP) \cite{zhao2017dependent}. They also prove that many attractive properties of DP, like post-processing and composition guarantees, also hold for BDP. Liu et al. \cite{liu2016dependence} consider a different privacy definition that they also term dependent differential privacy; however, their definition is quite distinct, as it doesn't imply DP \cite{zhao2017dependent}. \todolong{Add more papers? Fang-Yi mentioned \cite{naim2019off}, which is a very interesting but different application of correlated privacy}

As far as mechanisms, the original BDP paper considers a mechanism for the sum query, with data drawn from a Gaussian query model \cite{yang2015bayesian}. Our setting is very different from this. However, they also show that the adversary with the least prior knowledge is the hardest to protect against with positive data correlation; we employ a similar result in our setting. Song et al. provide a very general mechanism that guarantees any privacy for any definition in the Pufferfish framework \cite{song2017pufferfish}. However, their model may be computationally intractable, and must be re-run (with additional privacy loss) for multiple queries. Zhao et al. provides a very general reduction theorem which explains how $\eps$-BDP is implied by a lower $\eps'$-DP. This result, while very powerful, does not produce optimal noise-privacy tradeoffs, as we explore in section 3. 

To best of the authors' knowledge, this is the first paper with an explicit mechanism for distributed, non-interactive privacy in correlated settings.
% \begin{enumerate}
%     \item Overall, no work on non-interactive privacy with correlated data.
%     \item Talk about various privacy definitions:
%     \begin{enumerate}
%         \item DP: Not good because the data is correlated and all belongs to a single individual.
%         \item Coupled-Worlds: not good when the data all belongs to a single individual.
%         \item DDP (2016): Seems like they protect against only the ``strongest'' BDP adversary. Relies on computing a dependence coefficient between all data points in the model? Needlessly complicated?
%         \item DDP (2017): they claim that they don't assume that adversary knows the correlation (their definition works regardless of whether the adversary knows the correlation). \textcolor{red}{Need to look more into this. Their work seems very thorough/well-motivated. Maybe empirical comparison?}
%     \end{enumerate}
%     \item ~\cite{song2017pufferfish}: provides a mechanism, but is query based
%     \item ~\cite{yang2015bayesian}: Assumes a Gaussian correlation model, which is not good for our applications (time series data)
%     \item \cite{naim2019off} consider a privacy notion for a single person.  We can include it in the related work.
% \end{enumerate}

% To do this, we will use Markov Random Fields as models for the data of each agent in a social network, and Pufferfish privacy as the privacy objective. We investigate a generalized random response mechanism, which has the added benefit of guaranteeing ``local" Pufferfish privacy (even the curator need not know agents' true data).  We show a trade-off between the differential privacy achievable (when one ignores correlations) and the Pufferfish privacy achievable (when correlations are taken into account). Specifically, we show that $\eps$-differential privacy requires less noise than $\eps$-Pufferfish privacy, and also that $\eps$-differential privacy fails when the adversary has knowledge about the data distribution. We will also identify the trade-offs of algorithmic efficiency and different privacy guarantees.

==> Pufferfish Privacy for Sanitized Databases/introduction-shorter.tex <==


\section{Introduction}
In the literature of privacy, differential privacy (DP)~\cite{dwork2014algorithmic} is the most popular model. An algorithm is differentially private if its outputs with and without any individual's data are (nearly) indistinguishable. It guards against what an adversary learns about an agent \textit{due directly} to that agent's participation. But this does not offer guarantees on how much an adversary can infer about personal data from the perturbed output.
Specifically, with correlated data, %DP's guarantee is insufficient, as
an adversary understanding the correlation can bolster inference significantly~\cite{Kifer2011no}. Real world data typically exhibits natural correlation structures.  Social networks mediate interactions and influence which often lead to strongly correlated personal attributes.   Similarly, spatial and temporal proximity leads to strong correlations in data from sensors recorded as discretized time series. Examples include data from human mobility traces, power grids, health data from personal wearable devices, and US census data.
In many applications the correlation structure can be learned from historical data and so should be assumed to be public knowledge. Let the \textit{correlated advantage} be how much an adversary can infer about private data from the perturbed output, given explicit knowledge of the correlation structure. We want a privacy 
%definition and 
mechanism that bounds the correlated advantage.  

To incorporate correlated data, the Pufferfish framework, proposed by \citet{kifer2014pufferfish}, allows for robust privacy guarantees based on a specified data generation model and secret pairs.
Bayesian differential privacy (BDP), initially proposed by \citet{yang2015bayesian}, is an instantiation of the Pufferfish privacy framework and a generalization of differential privacy. The distinction between DP and BDP is most salient when comparing which adversaries they protect against. DP protects against adversaries who know all but one tuple, while BDP quantifies over adversaries who know arbitrarily many tuples. As an example, suppose we are trying to protect Alice's time series data. Differential privacy guarantees %\textit{only} 
that someone who knows Alice's location at all but one time step will not learn very much by analyzing the sanitized data set (their posterior after seeing the sanitized data will not change much)~\cite{yang2015bayesian}. BDP guarantees that, regardless of what the adversary knows about Alice's mobility data, they will not learn much by analyzing the sanitized data set.\footnote{Notice that when the data at each time step is independent, BDP reduces to DP; the adversary's knowledge of Alice's location at time $x_i$ is irrelevant to their knowledge of Alice's location at time $x_j$.} Presumably, Alice is probably not very interested in protecting her data only against an adversary who knows almost all of it. Analogously, we hope to achieve privacy guarantees that do not depend on how many data points the adversary knows.
\subsection{Our Contribution}

Our main theoretical contribution is providing a mechanism for achieving BDP when the data is drawn from a binary Markov chain. We focus on \textit{non-interactive} mechanisms, which return ``sanitized'' (i.e. noisy) estimates of the real database. These are called non-interactive since the sanitized databases can be queried offline without further privacy loss; in contrast, query-based mechanisms must be rerun with additional privacy losses for each query. In order to achieve \textit{local} privacy guarantees, our primary mechanism adds independent noise to each tuple. Local privacy means that no centralized curator needs to have access to the agents' true data. Instead, the owners of each tuple can privately sanitize their entry before submission, which would be ideal for IoT settings. When privacy guarantees are framed in terms of trust or persuasive power, this property is extremely attractive.\footnote{Though we mostly focus on the setting where every tuple belongs to one individual, our mechanism is still applicable to the conventional setting.} 

Our model is simple yet fundamental; we represent data correlations via Markov chains, and these preliminary results consider only binary state spaces. We assume that the data is \textit{positively} correlated, as in the case of location data, where an individual is more likely to stay in the same location than leave (given a fine-enough time scale). We improve on the state-of-the-art BDP mechanism and show that our mechanism provides the \emph{optimal} noise-privacy tradeoffs (among local/independent noise mechanisms) up to negligible factors. This is significant because the previous general results only provide a sufficient bound on the noise~\cite{liu2016dependence, zhao2017dependent}. The main challenge with finding an exact bound is describing how the privacy loss evolves through the Markov chain. We also consider a mechanism which adds \textit{correlated} noise to the data, but find no additional improvement to noise-privacy tradeoffs. Lastly, we perform experiments on real and synthetic data. 
We first demonstrate that DP does not bound the correlated advantage, by providing a concrete, correlation aware attack that more than doubles the DP bound.
Further, even on real data that is not entirely Markovian, a neural network adversary, using Long Short Term Memory (LSTM) models, cannot surpass our mechanism's privacy bounds, suggesting that our mechanism is \textit{robust} to varying correlation structures in practice.

\subsection{Related Work}
The limitation of differential privacy with correlated data has been pointed out in different contexts~\cite{Kifer2011no, chen2014correlated, yang2015bayesian, song2017pufferfish,zhao2017dependent,he2014blowfish,zhu2014correlated}. As a result, there have been new correlation-aware privacy definitions in recent years. \citet{zhao2017dependent} consider a definition equivalent to BDP that they term \emph{dependent differential privacy}. Their proofs show that many attractive properties of DP, like post-processing and composition guarantees, also hold for BDP.  \citet{liu2016dependence} consider a different privacy definition that they also term dependent differential privacy; however, their definition is quite distinct, as it does not imply DP \cite{zhao2017dependent}.  \citet{naim2019off} consider a privacy definition rooted in information theory, that is more applicable to Internet privacy. 

As far as privacy preserving mechanisms, the original BDP paper considers a mechanism for the sum query, with data drawn from a Gaussian query model \cite{yang2015bayesian}. We model data generated from a Markov chain, so their mechanism does not apply.  \citet{song2017pufferfish} provide a very general mechanism along with guarantees for any privacy definition in the Pufferfish framework. However, their mechanism may be computationally heavy (e.g. it runs in $O(n^3)$ in our setting, while ours runs in time $O(n)$, for data of size $n$), and must be re-run (with additional privacy loss) for multiple queries. \citet{zhao2017dependent} provides a very general reduction theorem which explains how $\eps$-BDP is implied by a lower $\eps'$-DP. This result, while very powerful, does not produce optimal noise-privacy tradeoffs, as we explore in section 3. 

To the best of the authors' knowledge, this is the first paper with an explicit optimal mechanism for local, non-interactive privacy in correlated settings.

\smallskip\noindent\textbf{Roadmap} In Section 2, we review some basic definitions, and clearly differentiate the semantic guarantees of DP and BDP. In Section 3, we describe the noise-privacy tradeoffs of our mechanism, provide high level proof sketches, and briefly discuss a correlated noise variant of our mechanism. In Section 4, we run several experiments and compare with prior results. We show that $\eps$-DP requires less noise than $\eps$-BDP, and also experimentally evaluate how much privacy degrades when an adversary knows the data correlation structures. We then compare our noise-privacy tradeoffs with previous results, showing that we improve on the state-of-the-art. To round out our experiments, we evaluate our mechanism on real world heart rate data which may not be purely Markovian, which shows that our mechanism is robust to real world correlation patterns.

==> Pufferfish Privacy for Sanitized Databases/introduction.tex <==


\section{Introduction}
In the literature of privacy, differential privacy (DP)~\cite{dwork2014algorithmic} is the most popular model. An algorithm is differentially private if its outputs with and without any individual's data are (nearly) indistinguishable. It guards against what an adversary learns about an agent \textit{due directly} to that agent's participation. But this does not offer guarantees on how much an adversary can infer about personal data from the perturbed output.
Specifically, with correlated data, DP's guarantee is insufficient, as understanding the correlation can bolster inference significantly~\cite{Kifer2011no}. Real world data exhibits several natural correlation structures.  Social networks mediate interactions and influence which often lead to strongly correlated personal attributes.   Similarly, spatial and temporal proximity lead to strong correlations in data from sensors recorded as discretized time series. Some examples include data from human mobility traces, power grids, health data from personal wearable devices, and US census data.
In many applications the correlation structure can be learned from historical data and so should be assumed to be public knowledge. Let the \textit{correlated advantage} be how much an adversary can infer about private data from the perturbed output, given explicit knowledge of the correlation structure. We want a privacy definition and mechanism that bounds the correlated advantage.  

To incorporate correlated data, the Pufferfish framework, proposed by \citet{kifer2014pufferfish}, allows for robust privacy guarantees based on a specified data generation model and secret pairs.
Bayesian differential privacy (BDP), initially proposed by \citet{yang2015bayesian}, is an instantiation of the Pufferfish privacy framework and a strict generalization of differential privacy. The distinction between DP and BDP is most salient when comparing which adversaries they protect against. DP protects only against adversaries who know all but one tuple, while BDP simply quantifies over adversaries who know arbitrarily many tuples. As an example, suppose we are trying to protect Alice's time series data. Differential privacy guarantees \textit{only} that someone who knows Alice's location at all but one time step will not learn very much by analyzing the sanitized data set (their posterior after seeing the sanitized data will not change much)~\cite{yang2015bayesian}. BDP guarantees that, regardless of what the adversary knows about Alice's mobility data, they will not learn much by analyzing the sanitized data set.\footnote{Notice that when the data at each time step is independent, BDP reduces to DP; the adversary's knowledge of Alice's location at time $x_i$ is irrelevant to their knowledge of Alice's location at time $x_j$.} Presumably, Alice is not interested in protecting her data only against an adversary who knows almost all of it. Analogously, our privacy guarantee should not depend on how many data points the adversary knows.
\subsection{Our Contribution}

Our main theoretical contribution is providing a mechanism for achieving BDP when the data is drawn from a binary Markov chain.  We focus on \textit{non-interactive} mechanisms, which return ``sanitized'' (i.e. noisy) estimates of the real database. These are called non-interactive since the sanitized databases can be queried offline without further privacy loss; in contrast, query-based mechanisms must be rerun with additional privacy losses for each query. In order to achieve \textit{local} privacy guarantees, our primary mechanism adds independent noise to each tuple. Local privacy means that no centralized curator needs to have access to the agents' true data. Instead, the owners of each tuple can privately sanitize their entry before submission, which would be ideal for IoT settings. When privacy guarantees are framed in terms of trust or persuasive power, this property is extremely attractive.\footnote{Though we mostly focus on the setting where every tuple belongs to one individual, our mechanism is still applicable to the conventional setting.} 

Our model is simple yet fundamental; we represent data correlations via Markov chains, and these preliminary results consider only binary state spaces. We assume that the data is \textit{positively} correlated, as in the case of location data, where an individual is more likely to stay in the same location than leave (given a fine-enough time scale). We improve on the state-of-the-art BDP mechanism and show that our mechanism provides the \emph{optimal} noise-privacy tradeoffs (among local/independent noise mechanisms) up to negligible factors. This is significant because the previous general results only provide a sufficient bound on the noise~\cite{liu2016dependence, zhao2017dependent}. The main challenge with finding an exact bound is describing how the privacy loss evolves through the Markov chain. We also consider a mechanism which adds \textit{correlated} noise to the data, but find no additional improvement to noise-privacy tradeoffs. Lastly, we perform experiments on real and synthetic data. 
We first demonstrate that DP does not bound the correlated advantage, by providing a concrete, correlation aware attack that more than doubles the DP bound.
Further, even on real data that is not entirely Markovian, a neural network adversary, using Long Short Term Memory (LSTM) models, cannot surpass our mechanism's privacy bounds, suggesting that our mechanism is \textit{robust} to varying correlation structures in practice.

\subsection{Related Work}
There exists a large body of work regarding the limitation of differential privacy with correlated data.\footnote{See \cite{Kifer2011no, chen2014correlated, yang2015bayesian, song2017pufferfish,zhao2017dependent,he2014blowfish,zhu2014correlated} for examples in various contexts.} As a result, there have been many new correlation-aware privacy definitions in recent years. \citet{zhao2017dependent} consider a definition equivalent to BDP that they term \emph{dependent differential privacy}. Their proofs show that many attractive properties of DP, like post-processing and composition guarantees, also hold for BDP.  \citet{liu2016dependence} consider a different privacy definition that they also term dependent differential privacy; however, their definition is quite distinct, as it does not imply DP \cite{zhao2017dependent}.  \citet{naim2019off} consider a privacy definition rooted in information theory, that is more applicable to Internet privacy. 

As far as privacy preserving mechanisms, the original BDP paper considers a mechanism for the sum query, with data drawn from a Gaussian query model \cite{yang2015bayesian}. We model data generated from a Markov chain, so their mechanism does not apply.  \citet{song2017pufferfish} provide a very general mechanism along with guarantees for any privacy definition in the Pufferfish framework. However, their mechanism may be computationally intractable (e.g. it runs in $O(n^3)$ in our setting, while ours runs in time $O(n)$), and must be re-run (with additional privacy loss) for multiple queries. \citet{zhao2017dependent} provides a very general reduction theorem which explains how $\eps$-BDP is implied by a lower $\eps'$-DP. This result, while very powerful, does not produce optimal noise-privacy tradeoffs, as we explore in section 4. 

To the best of the authors' knowledge, this is the first paper with an explicit optimal mechanism for local, non-interactive privacy in correlated settings.

\smallskip\noindent\textbf{Roadmap} In section 2, we review some basic definitions, and clearly differentiate the semantic guarantees of DP and BDP. In section 3, we describe the noise-privacy tradeoffs of our mechanism, provide high level proof sketches, and briefly discuss a correlated noise variant of our mechanism. In section 4, we run several experiments and compare with prior results. We show that $\eps$-DP requires less noise than $\eps$-BDP, and also experimentally evaluate how much privacy degrades when an adversary knows the data correlation structures. We then compare our noise-privacy tradeoffs with previous results, showing that we improve on the state-of-the-art. To round out our experiments, we evaluate our mechanism on real world heart rate data which may not be purely Markovian, which shows that our mechanism is robust to real world correlation patterns.

==> introduction-6-7-8pm.tex <==
\section{Introduction}
In the literature of privacy, differential privacy (DP)~\cite{dwork2014algorithmic} is the gold standard. An algorithm is differentially private if its outputs with and without any individual's data are indistinguishable. But there are numerous settings in which the semantic guarantees of differential privacy either aren't meaningful or are insufficient. Bayesian differential privacy (BDP)~\cite{yang2015bayesian} is a strict generalization of differential privacy that is applicable in many of these settings. However, BDP is more technically challenging to work with; our main theoretical contribution is providing a mechanism for achieving BDP when the data is drawn from a binary Markov chain. In this regard, we improve on the state-of-the-art BDP mechanism and show that our mechanism provides the optimal noise-privacy tradeoffs up to negligible factors. We also consider a mechanism which adds \textit{correlated} noise to the data, but find no improvement to noise-privacy tradeoffs. Lastly, we perform experiments on synthetic data that details when DP is insufficient, and experiments on real data to show that our mechanism works well in practice even when the underlying distribution is not a simple Markov chain. We start by arguing the need for stronger privacy than DP.

\subsection{Privacy Definitions}

Differential privacy forms privacy guarantees \textit{without} a model for how the data is generated. A differentially private mechanism guarantees that the probability ratio of observing any single output by applying the mechanism to two \textit{neighboring} databases is small, where two databases are neighbors if they differ in exactly one data point. Importantly, the probability here is only taken over the randomness of the mechanism, since there's no model for data generation. However, if an adversary has reasonable background knowledge regarding the data distributions, it may be the case that an $\eps$-differentially private mechanism will produce an output that is disproportionately more likely given one of two neighboring datasets. So in examples where adversaries can reasonably infer the data correlation model (e.g. US census data), differential privacy will \textit{not} prevent these adversaries from learning tuples. 

This limitation of DP is well understood;~\cite{dwork2014algorithmic} reframes this limitation in terms of the \textit{semantic} guarantee that DP provides. Suppose you are a medical researcher tasked with convincing users to divulge sensitive health data, which will then be published online. Differential privacy, according to the semantic interpretation, can be used as a \textit{tool} to encourage participation. Individuals, who can only control their own participation in the study, know that they will receive minimal harm \textit{directly tied} to their participation in the study. Viewed this way, DP is an entirely end-user focused persuasive tool. However, an ethical researcher would not only like to persuade users to participate, but also to understand and limit the harms caused by the study itself. DP answers the question of whether a single user ought to participate; BDP answers the question of whether the study ought to be performed. Put this way, BDP and similar privacy frameworks can be viewed as mechanism design for social good. Another way to frame this is that BDP persuades the researcher to publish their collected data, by more comprehensively limiting the harms to any study participant.

When the database consists of records that each belong to different individuals, DP can still be a reasonable choice (e.g. if the study could significantly help the participants). However, when considering data from a single individual, such as the mobility data of a single person, DP does not provide any meaningful guarantees. The distinction here is most salient when comparing which adversaries DP and BDP protect against. Suppose we are trying to protect Alice's time series data. Differential privacy guarantees \textit{only} that someone who knows Alice's location at all but one time step will not learn very much by analyzing the sanitized data set (their posterior after seeing the sanitized data won't change much)~\cite{yang2015bayesian}. BDP guarantees that regardless of how much the adversary knows, they won't learn much by analyzing the sanitized data set. Presumably, Alice is not interested in protecting her data only against an adversary who knows almost all of it. Analogously, our privacy guarantee should not depend on how many data points the adversary knows.\footnote{Notice that when the data at each time step is independent, BDP reduces to DP; the adversary's knowledge of Alice's location at time $x_i$ is irrelevant to their knowledge of Alice's location at time $x_j$.}

\subsection{Our Contribution}

BDP is an instantiation of the Pufferfish privacy framework~\cite{kifer2014pufferfish}, a broad framework that allows us for customizable, robust privacy guarantees. We focus on providing \textit{non-interactive} mechanisms, which return ``sanitized'' (i.e. noisy) estimates of the real database. These are called non-interactive since the sanitized databases can be queried offline without further privacy loss; in contrast, query-based mechanisms must be rerun with additional privacy losses for each query. Our primary mechanism adds independent noise to each state; because of this, our mechanism achieves \textit{distributed}, or local, privacy guarantees. This means that no centralized curator need have access to the agents' true data. Instead, the owners of each tuple can privately sanitize their entry before submission. When privacy guarantees are framed in terms of trust or persuasive power, this property is extremely attractive.\footnote{Though we mostly focus on the setting where every tuple belongs to one individual, our mechanism is still applicable to the conventional setting.} 
% The main challenge in the setting of correlated data is a lack of suitable mechanisms. Recent advances~\cite{song2017pufferfish} provide a Pufferfish private mechanism under the query setting: given a functional query, e.g., counting the number of smokers, the mechanism's report is private and close to the real value. That mechanism has two main limitations: (1) it is computationally intractable, and (2) the mechanism cannot handle adaptive queries, but instead must be rerun (and lose additional privacy guarantees) for each query. For this reason, we design efficient \textit{non-interactive} mechanisms, that will release a noisy estimate of the real database (to make the reports reusable).

Our model is relatively simple; we represent data correlations via Markov chains, and these preliminary results consider only binary state spaces. We assume that the data is \textit{positively} correlated, as in the case of location data, where an individual is more likely to stay in the same location than leave (given a fine-enough time scale). 
\paragraph{Roadmap} In Section 2, we review the definition of BDP, and apply it to the context of our problem. In Section 3, we first state our main theorem, which describes the noise-privacy tradeoffs of our mechanism. We show that $\eps$-differential privacy requires less noise than $\eps$-BDP, but also experimentally evaluate how much privacy degrades when an adversary has knowledge about the data distribution. (show concrete attack on DP with synthetic data). We then compare our noise-privacy tradeoffs with previous results, showing that we improve on the state-of-the-art. To round out our experiments, we evaluate our mechanism on real heart rate data, showing that the Markov chain modelling assumption cannot be exploited by an LSTM deep learning adversary. We also measure the accuracy of basic metrics on the sanitized data.

In Section 4, we prove our main theorem and also briefly discuss a mechanism which adds \textit{correlated} noise to the data. We find no improvement to the noise-privacy tradeoff, but \todolong{add some stuff about uses of the correlated noise mechanism, or say that it shows that our independent noise mechanism optimizes over a far large space of mechanisms.}

\subsection{Related Work}
In recent years, there have been many correlation-aware privacy definitions. We discuss a few of the most relevant definitions. Most of the definitions are instantiations of Pufferfish privacy ~\cite{kifer2014pufferfish}, a broad Bayesian framework. The most relevant is obviously Bayesian differential privacy, initially proposed by Yang et al.~\cite{yang2015bayesian}. They show that BDP is a very natural way to formulate a stronger privacy guarantee than DP, as BDP simply quantifies over adversaries with knowledge of any tuples, while DP only protects over adversaries who know all but one tuple. Zhao et al. consider an equivalent formulation that they term dependent differential privacy (DDP) \cite{zhao2017dependent}. They also prove that many attractive properties of DP, like post-processing and composition guarantees, also hold for BDP. Liu et al. \cite{liu2016dependence} consider a different privacy definition that they also term dependent differential privacy; however, their definition is quite distinct, as it doesn't imply DP \cite{zhao2017dependent}. \todolong{Add more papers? Fang-Yi mentioned \cite{naim2019off}, which is a very interesting but different application of correlated privacy}

As far as mechanisms, the original BDP paper considers a mechanism for the sum query, with data drawn from a Gaussian query model \cite{yang2015bayesian}. Our setting is very different from this. However, they also show that the adversary with the least prior knowledge is the hardest to protect against with positive data correlation; we employ a similar result in our setting. Song et al. provide a very general mechanism that guarantees any privacy for any definition in the Pufferfish framework \cite{song2017pufferfish}. However, their model may be computationally intractable, and must be re-run (with additional privacy loss) for multiple queries. Zhao et al. provides a very general reduction theorem which explains how $\eps$-BDP is implied by a lower $\eps'$-DP. This result, while very powerful, does not produce optimal noise-privacy tradeoffs, as we explore in section 3. 

To best of the authors' knowledge, this is the first paper with an explicit mechanism for distributed, non-interactive privacy in correlated settings.
% \begin{enumerate}
%     \item Overall, no work on non-interactive privacy with correlated data.
%     \item Talk about various privacy definitions:
%     \begin{enumerate}
%         \item DP: Not good because the data is correlated and all belongs to a single individual.
%         \item Coupled-Worlds: not good when the data all belongs to a single individual.
%         \item DDP (2016): Seems like they protect against only the ``strongest'' BDP adversary. Relies on computing a dependence coefficient between all data points in the model? Needlessly complicated?
%         \item DDP (2017): they claim that they don't assume that adversary knows the correlation (their definition works regardless of whether the adversary knows the correlation). \textcolor{red}{Need to look more into this. Their work seems very thorough/well-motivated. Maybe empirical comparison?}
%     \end{enumerate}
%     \item ~\cite{song2017pufferfish}: provides a mechanism, but is query based
%     \item ~\cite{yang2015bayesian}: Assumes a Gaussian correlation model, which is not good for our applications (time series data)
%     \item \cite{naim2019off} consider a privacy notion for a single person.  We can include it in the related work.
% \end{enumerate}

% To do this, we will use Markov Random Fields as models for the data of each agent in a social network, and Pufferfish privacy as the privacy objective. We investigate a generalized random response mechanism, which has the added benefit of guaranteeing ``local" Pufferfish privacy (even the curator need not know agents' true data).  We show a trade-off between the differential privacy achievable (when one ignores correlations) and the Pufferfish privacy achievable (when correlations are taken into account). Specifically, we show that $\eps$-differential privacy requires less noise than $\eps$-Pufferfish privacy, and also that $\eps$-differential privacy fails when the adversary has knowledge about the data distribution. We will also identify the trade-offs of algorithmic efficiency and different privacy guarantees.

==> introduction-shorter.tex <==


\section{Introduction}
In the literature of privacy, differential privacy (DP)~\cite{dwork2014algorithmic} is the most popular model. An algorithm is differentially private if its outputs with and without any individual's data are (nearly) indistinguishable. It guards against what an adversary learns about an agent \textit{due directly} to that agent's participation. But this does not offer guarantees on how much an adversary can infer about personal data from the perturbed output.
Specifically, with correlated data, %DP's guarantee is insufficient, as
an adversary understanding the correlation can bolster inference significantly~\cite{Kifer2011no}. Real world data typically exhibits natural correlation structures.  Social networks mediate interactions and influence which often lead to strongly correlated personal attributes.   Similarly, spatial and temporal proximity leads to strong correlations in data from sensors recorded as discretized time series. Examples include data from human mobility traces, power grids, health data from personal wearable devices, and US census data.
In many applications the correlation structure can be learned from historical data and so should be assumed to be public knowledge. Let the \textit{correlated advantage} be how much an adversary can infer about private data from the perturbed output, given explicit knowledge of the correlation structure. We want a privacy 
%definition and 
mechanism that bounds the correlated advantage.  

To incorporate correlated data, the Pufferfish framework, proposed by \citet{kifer2014pufferfish}, allows for robust privacy guarantees based on a specified data generation model and secret pairs.
Bayesian differential privacy (BDP), initially proposed by \citet{yang2015bayesian}, is an instantiation of the Pufferfish privacy framework and a generalization of differential privacy. The distinction between DP and BDP is most salient when comparing which adversaries they protect against. DP protects against adversaries who know all but one tuple, while BDP quantifies over adversaries who know arbitrarily many tuples. As an example, suppose we are trying to protect Alice's time series data. Differential privacy guarantees %\textit{only} 
that someone who knows Alice's location at all but one time step will not learn very much by analyzing the sanitized data set (their posterior after seeing the sanitized data will not change much)~\cite{yang2015bayesian}. BDP guarantees that, regardless of what the adversary knows about Alice's mobility data, they will not learn much by analyzing the sanitized data set.\footnote{Notice that when the data at each time step is independent, BDP reduces to DP; the adversary's knowledge of Alice's location at time $x_i$ is irrelevant to their knowledge of Alice's location at time $x_j$.} Presumably, Alice is probably not very interested in protecting her data only against an adversary who knows almost all of it. Analogously, we hope to achieve privacy guarantees that do not depend on how many data points the adversary knows.
\subsection{Our Contribution}

Our main theoretical contribution is providing a mechanism for achieving BDP when the data is drawn from a binary Markov chain. We focus on \textit{non-interactive} mechanisms, which return ``sanitized'' (i.e. noisy) estimates of the real database. These are called non-interactive since the sanitized databases can be queried offline without further privacy loss; in contrast, query-based mechanisms must be rerun with additional privacy losses for each query. In order to achieve \textit{local} privacy guarantees, our primary mechanism adds independent noise to each tuple. Local privacy means that no centralized curator needs to have access to the agents' true data. Instead, the owners of each tuple can privately sanitize their entry before submission, which would be ideal for IoT settings. When privacy guarantees are framed in terms of trust or persuasive power, this property is extremely attractive.\footnote{Though we mostly focus on the setting where every tuple belongs to one individual, our mechanism is still applicable to the conventional setting.} 

Our model is simple yet fundamental; we represent data correlations via Markov chains, and these preliminary results consider only binary state spaces. We assume that the data is \textit{positively} correlated, as in the case of location data, where an individual is more likely to stay in the same location than leave (given a fine-enough time scale). We improve on the state-of-the-art BDP mechanism and show that our mechanism provides the \emph{optimal} noise-privacy tradeoffs (among local/independent noise mechanisms) up to negligible factors. This is significant because the previous general results only provide a sufficient bound on the noise~\cite{liu2016dependence, zhao2017dependent}. The main challenge with finding an exact bound is describing how the privacy loss evolves through the Markov chain. We also consider a mechanism which adds \textit{correlated} noise to the data, but find no additional improvement to noise-privacy tradeoffs. Lastly, we perform experiments on real and synthetic data. 
We first demonstrate that DP does not bound the correlated advantage, by providing a concrete, correlation aware attack that more than doubles the DP bound.
Further, even on real data that is not entirely Markovian, a neural network adversary, using Long Short Term Memory (LSTM) models, cannot surpass our mechanism's privacy bounds, suggesting that our mechanism is \textit{robust} to varying correlation structures in practice.

\subsection{Related Work}
The limitation of differential privacy with correlated data has been pointed out in different contexts~\cite{Kifer2011no, chen2014correlated, yang2015bayesian, song2017pufferfish,zhao2017dependent,he2014blowfish,zhu2014correlated}. As a result, there have been new correlation-aware privacy definitions in recent years. \citet{zhao2017dependent} consider a definition equivalent to BDP that they term \emph{dependent differential privacy}. Their proofs show that many attractive properties of DP, like post-processing and composition guarantees, also hold for BDP.  \citet{liu2016dependence} consider a different privacy definition that they also term dependent differential privacy; however, their definition is quite distinct, as it does not imply DP \cite{zhao2017dependent}.  \citet{naim2019off} consider a privacy definition rooted in information theory, that is more applicable to Internet privacy. 

As far as privacy preserving mechanisms, the original BDP paper considers a mechanism for the sum query, with data drawn from a Gaussian query model \cite{yang2015bayesian}. We model data generated from a Markov chain, so their mechanism does not apply.  \citet{song2017pufferfish} provide a very general mechanism along with guarantees for any privacy definition in the Pufferfish framework. However, their mechanism may be computationally heavy (e.g. it runs in $O(n^3)$ in our setting, while ours runs in time $O(n)$, for data of size $n$), and must be re-run (with additional privacy loss) for multiple queries. \citet{zhao2017dependent} provides a very general reduction theorem which explains how $\eps$-BDP is implied by a lower $\eps'$-DP. This result, while very powerful, does not produce optimal noise-privacy tradeoffs, as we explore in section 3. 

To the best of the authors' knowledge, this is the first paper with an explicit optimal mechanism for local, non-interactive privacy in correlated settings.

\smallskip\noindent\textbf{Roadmap} In Section 2, we review some basic definitions, and clearly differentiate the semantic guarantees of DP and BDP. In Section 3, we describe the noise-privacy tradeoffs of our mechanism, provide high level proof sketches, and briefly discuss a correlated noise variant of our mechanism. In Section 4, we run several experiments and compare with prior results. We show that $\eps$-DP requires less noise than $\eps$-BDP, and also experimentally evaluate how much privacy degrades when an adversary knows the data correlation structures. We then compare our noise-privacy tradeoffs with previous results, showing that we improve on the state-of-the-art. To round out our experiments, we evaluate our mechanism on real world heart rate data which may not be purely Markovian, which shows that our mechanism is robust to real world correlation patterns.
